Eye Gaze as a Signal for Conveying User Attention in Contextual AI Systems

Advanced multimodal AI agents can now collaborate with users to solve challenges in the world. Yet, these emerging contextual AI systems rely on explicit communication channels between the user and system. We hypothesize that implicit communication of the user's interests and intent would reduce friction and improve user experience when collaborating with AI agents. In this work, we explore the potential of wearable eye tracking to convey signals about user attention. We measure the eye tracking signal quality requirements to effectively map gaze traces to physical objects, then conduct experiments that provide visual scanpath history as additional context when querying vision language models. Our results show that eye tracking provides high value as a user attention signal and can convey important context about the user's current task and interests, improving understanding of contextual AI agents.

==> planning.tex <==
\newpage
\section*{PLANNING / OUTLINING}

\textbf{Publication Narrative}
\begin{outline}
    \1 Overview
        \2 It is hypothesized that eye gaze is the strongest indicator of a user's attention.
            \3 capturing what objects they are interested in, cognitive load, etc.
        \2 We investigate eye tracking as a mode for capturing a user's attention.
        \2 We quantify the expected eye tracking error requirements to detect intersections with physical objects.
        \2 We show initial benefits for including eye gaze context in contextual AI systems.
    \1 Related literature
        \2 Eye movements encode cognitive processes of scene perception.
            \3 Objects entering / leaving peripersonal space (\href{https://docs.google.com/document/d/1OAa3BbKrZ0tp2w21b3jMOShmPjgfZFuIS-TRGBk696s/edit?tab=t.0#heading=h.6kwwrcva4vwt}{written up here}).
            \3 Charlie's works investigating scan paths / temporal gaze information.
        \2 Eye tracking as a selection mechanism:
            \3 citations on usage in VR and AR studies.
        \2 World-facing contextual AI:
            \3 Multimodal querying with images / video.
            \3 Devices like project Aria (and associated datasets) which advance AI scene understanding of physical world.
        \2 Eye tracking contextual AI prototypes:
            \3 GazeGPT cropping scene information to the fixated object.
            \3 G-VOILA prototypes the concept using gaze scanpath information and replacing ambiguous pronouns in querying.
            \3 mention lack of analysis regarding the requirements for eye tracking to be effective in such systems.
    \1 Evaluation methodology
        \2 Aria digital twins dataset.
        \2 Interaction spaces (these are simplified, don't incorporate the focus heuristic in this paper).
            \3 Human-object interactions during physical interactions.
            \3 Distributed sizes of objects within 1 meter of the user.
            \3 within 2 meters of the user.
        
    \1 Evaluate eye tracking signal quality.
        \2 Sizes of objects when within each interaction space.
        \2 Relationship between an object's physical size and an object's visual size (should be pretty consistent).
        \2 But also looking at the distribution of objects that the user fixates on to see a natural distribution of object sizes in household scenarios.
        
    \1 Contextual AI experiments.
        \2 Experiments to evaluate the impact of various eye tracking capture metrics to end-to-end AI applications and whether information encoded in gaze makes a significant impact.
        \2 Experiment 1: predicting the user's attention (what am I looking at?)
            \3 connects to Charlie's prior work evaluating scanpaths and temporal patterns contained in gaze.
        \2 Experiment 2: predicting what a user will interact with based on scanpath history.
            \3 ground truth label is a hand-object interaction set to occur within 1 second.
        \2 Experiment 3: using projected gaze point to crop image contents, narrowing the point of focus.
            \3 Setup comparisons to both experiment 1 and experiment 2's base cases.

    \1 Discussion
        \2 Eye tracking has a clear role in contextual AI applications
        \2 Using eye tracking to supply contextual information is bottlenecked by the size of content the user is looking at
        \2 Over a range of household scenarios, we estimate the distribution of object sizes to be X Y and Z
        
\end{outline}

==> sections/methodology.tex <==
\section{Methodology}

To better understand ET's role in future contextual AI systems, we first estimate the ET signal quality needed for accurate gaze-based selection of physical objects.  Next, to measure the ability of AI agents to incorporate ET context, we experiment with end-to-end contextual AI tasks.  We inject contextual cues derived from the user's eye gaze into VLM queries, improving the model's ability to understand user attention and current actions.

\subsection{Eye tracking requirements for registering nearby objects}

Contextual AI models that collaborate with users would benefit from knowledge of users' real-world interests.  ET is a promising signal to capture the user's attention, both at one point in time~\cite{konrad_gazegpt_2024}, or continuously to build historical context.  We hypothesize that the visual angle subtended by objects that users ``look at'' defines a lower bound on ET signal accuracy.  By measuring the visual angle expressed by nearby objects, we can approximate the ET accuracy required to consistently track a user's point of focus.

To investigate accuracy requirements, we analyze objects that are nearby in the user's field of view (FOV) during daily household tasks, then relate the object size statistics to ET signal quality requirements.  Because we expect humans and AI agents to collaborate in daily life, it is important for the ET system to achieve an accuracy which allows consistent, accurate attention modeling in a broad set of scenarios~\cite{feit2017toward}.  Individuals are far more likely to look at or interact with objects in the immediate vicinity~\cite{ballendat_proxemic_2010}, so we constrain this analysis to objects which are nearby candidates for interaction.

\subsubsection{Dataset}

For our analyses, we use a subset of the Aria Digital Twins (ADT) dataset~\cite{pan_adt_2023}.  The ADT dataset contains egocentric recordings of daily-life tasks in indoor environments.  We analyze single-participant recordings in the fully furnished apartment scene (93 recordings), totaling $\sim$3 hours of footage.  Designed to model real-world household scenarios, these recordings span the following tasks:  decorating, cooking, working, cleaning, and object examination.

In addition to the ET signal (median error $= 1.5\degree$) provided by Project Aria glasses~\cite{engel_aria_2023}, the ADT dataset contains ground-truth information about physical objects in the scene.  Each object's position, orientation, bounding box, and segmentation region is tracked and available throughout a recording, with median tracking error of $5 mm$.  This ground-truth data uniquely enables us to analyze object visual statistics at a fine scale, detect human-object interactions, and accurately place gaze on objects.  396 household objects are tracked in the dataset, with varying presence across different tasks and recordings.

\subsubsection{Object visual size in relation to eye tracking error}

\begin{figure}[t]
 \centering
 \includegraphics[width=0.5\linewidth]{figures/segment_illustration_flat.png}
 \caption{Illustration of eye tracking spatial error and object visual size measurements.  As an average case measurement, object segmentation area can be mapped to a circular region, with the radius reflecting the eye tracking accuracy requirement (\textcolor{red}{thin bars}).  Alternatively, $1 / 2$ minor axis span $L_{min}$ (\textcolor{red}{thick bars}) is a tighter bound for measuring non-uniform objects.}
 \label{fig:et_relationship}
\end{figure}

ET spatial error is the measured bias between the ground truth and estimated gaze positions.  This error persists following techniques such as ET calibration and fixation detection.  We measure spatial error as an angular offset between the user's true gaze point and computed value.  We wish to approximate the influence of ET spatial error in placing fixations on object, to better inform how reliably an ET system could convey a user's attention on world objects.

Our metrics to predict ET accuracy needs are derived from object visual size, the visual angle spanned by the object relative to the user's FOV.  Visual size is related to both the physical size of an object and its distance from the user.  We approximate object visual size from the total segmentation area $A_{{}_{seg}}$ of an object in a linear camera model (measuring degrees$^2$ occupied by the object).  To convey visual size against an ET error requirement $err_{{}_{ET}}$, we convert visual size to the approximate \textbf{radius} of the object. $err_{{}_{ET}} \ \leq \ \sqrt{A_{{}_{seg}} / \pi}$.  This inequality approximates an \textbf{average case} need for ET error requirement, and is valid when objects have roughly uniform dimensions.  To account for non-uniform objects, we compute a more \textbf{conservative} ET error as $1 / 2$ the \textbf{minor axis} span $L_{min}$ of the object's segmentation region: $err_{{}_{ET}\ low} \ \leq \ 1 / 2 \ L_{min}$.  \autoref{fig:et_relationship} illustrates these metrics and the relationship between ET error requirements and object visual size.

\subsubsection{Protocol}

We approximate the ET requirements for daily use by observing the household tasks being performed in the ADT dataset~\cite{pan_adt_2023}.  We measure the distributions of object visual sizes for $err_{{}_{ET}}$ and $err_{{}_{ET}\ low}$.  To better inform various contextual AI applications, we specify the ET requirements across different interaction spaces, namely:
\begin{enumerate}  [topsep=0pt]
    \item \textbf{Near-field objects:} all objects within 1 meter of the participants.
    \item \textbf{Mid-field objects:} all objects between 1 - 2 meters of the participants.
    \item \textbf{Interacted objects:} all objects being physically interacted with (held, pressed, pushed, etc.) by the participants, with a start / stop padding of 1 second for the interaction.
    \item \textbf{Fixated objects:} all objects within 2 meters fixated on by participants' gaze as they navigate the scenes.
\end{enumerate}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/query_example.png}
    \caption{An example query to the VLM for E1.  The additional context from fixation history is highlighted in red; We vary the amount of context given to the model to measure how this context influences model understanding.}
    \label{fig:query_example}
\end{figure}

\subsection{Contextualizing vision-language model queries with eye tracking information}

To begin to explore the value that ET signals can provide in contextual AI systems, we model experiments which reflect potential end-to-end contextual AI systems.  In these experiments, we build up historical context by creating timelines of past fixations on physical objects.  We include this context in VLM queries and measure the positive impacts on model understanding.  Our baseline comparison is a VLM query which uses only the egocentric image as added context (similar to a Ray-Ban Meta or Google Ask Photos query).

We use the Meta Llama 3.2 90B VLM\footnote{\url{https://ai.meta.com/blog/llama-3-2-connect-2024-vision-edge-mobile-devices/}}~\cite{grattafiori_llama_2024} as our contextual AI agent.  We add context to queries with an egocentric image and additional prompting.  In both experiments, the agent is constrained via JSON to respond with one option from all currently visible objects, as we are operating under the pretense that in a full system, an object recognition / scene understanding model would be available.  Note that this VLM is not fine-tuned, and that a model tuned for egocentric image understanding and / or for a specific task would likely see improved results.  Yet, these experiments indicate the added value when incorporating ET contextual information.

\subsubsection{E1: ``What am I looking at?" with historical context.}

In this experiment, we pose the question ``what am I looking at?"  This experiment serves as a benchmark for the effect that prior eye gaze context serves in improving image understanding.  We first detect and localize fixations on objects\footnote{We use a velocity-thresholding algorithm at 100$\degree$ per second~\cite{salvucci_fixations_2000}, to account for the relatively low sampling rate of Project Aria glasses (30Hz)~\cite{engel_aria_2023}.  We only consider fixations $\geq$ 150 ms for analysis.}, then perform uniform random sampling across each recording in the ADT dataset to analyze 919 image frames which each contain at least 10 prior fixations.  At each sample, we make multiple queries, varying the number of prior fixations supplied as context to the VLM, between 0 - 10.  An example prompt set can be seen in~\autoref{fig:query_example}.

\subsubsection{E2: "What am I going to interact with?" with historical context.}

We query the VLM ``what am I going to interact with?" while again varying the amount of gaze context.  In this experiment, we supply the image from a current fixation, where a physical interaction is guaranteed to occur within the next second and at least 10 prior fixations exist (237 distinct image frames).  The vast majority of physical interactions in ADT are grasping, pushing, and pulling with hands.  This task models the use of ET as supporting context for user action understanding and prediction.

% \subsubsection{E3: Gaze-based context cropping.}

% In this experiment, we pose a similar question to E1 (``What am I looking at?"), but instead of providing historical context, we use the eye tracking signal to narrow down the visible region of the image supplied to the model.  This experiment models ET's efficacy in narrowing contextual image cues, preventing misunderstandings from objects which are not near the user's current point of gaze.  We then perform an ablation where we artificially degrade the eye tracker's accuracy, adding noise in a random direction before cropping and querying the VLM.

==> sections/results.tex <==
\section{Results}

\subsection{Eye tracking accuracy requirements}
\label{sec:accuracy_results}

\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{figures/vis_size.png}
    \caption{Eye tracking accuracy requirements to place gaze accurately within in the ADT dataset, where users performed household actions in an indoor environment~\cite{pan_adt_2023}  Near-field and mid-field measurements consider all objects present in the user's field of view, where interacted objects are being actively manipulated by the user, and fixated objects consider those being directly gazed at.}
    \label{fig:visual_sizes}
\end{figure}

The \textbf{near-field} ($\leq$ 1 meter) and \textbf{mid-field} (1 - 2 meters) measurements reflect the visual FOV occupied by \textit{every} object in the environment within the distance threshold.  Alternatively, the \textbf{interacted} measurement only aggregates objects when being manually interacted with, including picking up, pushing, pressing, etc.  \textbf{Fixation} measurements consider the objects within 2 meters at the time of fixation.  Considering ADT's household scenarios, the \textbf{interacted} and \textbf{fixation} categories reflect the distribution of objects likely to be of interest during daily tasks.

To estimate ET accuracy requirements, we computed the entire distribution of object visual sizes recorded in camera projection space. To place gaze on an object of average (projected) size 50\% of the time, we measure at the distribution's 50\% mark.  These measurements can help to inform system design; while 50\% reliability may be \textit{useful supporting context} in a broader contextual AI agent, a system relying heavily on ET may aim for higher coverage.  The distributions for each interaction scenario are seen in \autoref{fig:visual_sizes}.

Recall that we use angular \textbf{radius} to represent the \textbf{average case} ET requirements, and \textbf{minor axis} span as a more \textbf{conservative} measurement.  The accuracy of wearable ET devices is known to suffer in dynamic conditions~\cite{onkhar_tobii_2023}, yet recent devices remain quite accurate in unconstrained settings\footnote{\url{https://www.tobii.com/products/eye-trackers/wearables/tobii-pro-glasses-3}}\footnote{\url{https://pupil-labs.com/products/neon}}.  Assuming a device with $\leq 3 \degree$ accuracy during daily wear, our results indicate that the majority of fixated objects (radius average=$4.07\degree$; minor axis=$3.12\degree$), the majority of objects in the near-field (radius=$5.88\degree$; minor axis=$4.69\degree$), and nearly all interacted objects (radius=$10.81\degree$; minor axis=$9.10\degree$) are reliable for placing gaze on the correct object.  Conversely, objects in the mid-field (radius=$3.3\degree$; minor axis=$2.54\degree$) will be somewhat unreliable at this signal quality, where roughly half of objects are not able to be detected.

\subsection{Contextualized vision-language model queries}
\label{sec:vlm_queries}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/e1e2.png}
    \caption{Experiments where prior gaze fixation contents are supplied to a VLM along with egocentric images.  When many fixations given as context, the model can synthesize information between the image + gaze context to outperform a greedy baseline that only considers contents from the prompt. The error surfaces in light blue represent 95\% confidence intervals.}
    \label{fig:e1e2}
\end{figure}

Because we constrain the VLM model to respond by selecting from the list of all currently visible objects, these experiments are classification tasks where \textit{accuracy = correct selections / all trials}.  Cases where the VLM response failed to return parseable JSON ($<$1\% of trials) were discarded.

We compare against a number of baselines to see if the model effectively uses the context supplied.  These baselines implement simple heuristics on the image and gaze context.  The lowest performing baseline is random guessing among all visible objects.  We also implement random guesses from the list of previously fixated objects, and a greedy strategy which always chooses the most fixated object from a sequence of previously fixated objects.  Note these baselines still use context provided from ET, but make no attempt to synthesize with the egocentric image for better world understanding.

\subsubsection{E1: ``What am I looking at?"}

When querying the VLM only with the egocentric image as context, the model successfully predicts the current fixated object 10.3\% (95\% CI = [8.3\%, 12.3\%]) of the time (see \autoref{fig:e1e2} (left)).  While this surpasses random guessing from visible objects, it is quite low.  An effective strategy was to always return the immediately preceding fixation (left tail of Random (prior fixations) in \autoref{fig:e1e2}).  VLMs are not expected to excel at gaze prediction, as they are known to misinterpret context or hallucinate~\cite{cui_holistic_2023, leng_hallucinations_2024}.  However, including context from prior gaze greatly improves the model's ability to predict the current fixation, with a peak accuracy of 24.8\% (CI = [22.1\%, 27.7\%]) at 6 prior fixations.  The gaze context-based baselines slightly outperform the VLM with one or few prior fixations, reinforcing that current gaze is contingent on scanpath history~\cite{burlingham_laziness_2024, burlingham_scanpaths_2024}.  With more context (6+ fixations), the model begins to outperforms baselines, indicating that prior context and image contents are being synthesized, and the combination of contextual cues increase the model's performance.

\subsubsection{E2: ``What am I going to interact with?"}

E2 sees similar trends to E1; however, the more contextually-grounded task to predict the object of physical interaction sees greater benefit when including ET context. Clearly, prior eye gaze is a strong indicator for interaction, and by supplying historical gaze context, we can greatly improve the VLM's ability to understand the user's actions. We see a peak accuracy of 49.5\% (CI = [43\%, 56.1\%]). As evident by this and the stronger baseline performances, gaze is tightly coupled with the onset of interaction. Note that we query only at positive examples where an interaction does take place, and the inclusion of a null case could have led to the model raising false positives / negatives.


% \subsubsection{E3: Gaze-based context cropping}

% \NOTE{Holding space for this experiment.} \lipsum[1] \lipsum[2]
